Successive Cancellation Decoding of Single Parity-Check Product Codes: Analysis and Improved Decoding

A product code with single parity-check component codes can be described via the tools of a multi-kernel polar code, where the rows of the generator matrix are chosen according to the constraints imposed by the product code construction. Following this observation, successive cancellation decoding of such codes is introduced. In particular, the error probability of single parity-check product codes over binary memoryless symmetric channels under successive cancellation decoding is characterized. A bridge with the analysis of product codes introduced by Elias is also established for the binary erasure channel. Successive cancellation list decoding of single parity-check product codes is then described. For the provided example, simulations over the binary input additive white Gaussian channel show that successive cancellation list decoding outperforms belief propagation decoding applied to the code graph. Finally, the performance of the concatenation of a product code with a high-rate outer code is investigated via distance spectrum analysis. Examples of concatenations performing within $0.7$ dB from the random coding union bound are provided.

==> analysis_on_biMSC.tex <==
\subsection{Analysis over \mcc{the B-}AWGN Channel}
\label{sec:DE}

\mcc{Consider now transmission over \ac{B-AWGN} channel. Note that the \ac{B-AWGN} channel is symmetric, i.e.,$\W(y|0) = \W(-y|1)$\footnote{\mcc{A reader might assume \ac{BPSK} is adopted, where $0$ is mapped to $+1$ and $1$ to $-1$.}}, $\forall y\in\mathcal{Y}$. For symmetric channels, the error probability is independent of the codeword transmitted if linear codes are used\cite{Richardson:2008:MCT:1795974}. Then, w}e assume that all-zero codeword is transmitted for simplicity of the analysis. We write $L^{(i)}_{\G^{(m)}}(\vecy,\boldsymbol{0})$ to denote the the log-likelihood ratio of $u_i$ based on \eqref{eq:recurs_metric} where all the previous decisions are provided as zeros to the decoder, i.e.,
\begin{equation*}
	L^{(i)}_{\G^{(m)}}(\vecy,\boldsymbol{0}) \triangleq \log\frac{\W^{(i)}_{\G^{(m)}}(\vecy,\boldsymbol{0}|0)}{\W^{(i)}_{\G^{(m)}}(\vecy,\boldsymbol{0}|1)}.
\end{equation*}
Accordingly, we use $\ell^{(i)}_{\G^{(m)}}$ to denote the \ac{pdf} of \ac{RV} $L^{(i)}_{\G^{(m)}}(Y_1^n,\boldsymbol{0})$. The equation to compute the denisities are
\begin{equation}
	\ell^{(i)}_{\G^{(m)}} = \ell^{(j)}_{\G^{(m-1)}} \odot \left(\overset{t}{\mcc{\otimes}}\,\, \ell^{(j)}_{\G^{(m-1)}}\right) 
\end{equation}
where $j = \lfloor\frac{i-1}{k_m}\rfloor +1$, $t\triangleq i\mod k_m$, $\odot$ denotes the variable node convolution and $\overset{t}{\mcc{\otimes}}$ denotes the $t$-fold check node convolution with $\overset{1}{\mcc{\otimes}}\,\, \ell^{(j)}_{\G^{(m-1)}} \triangleq \ell^{(j)}_{\G^{(m-1)}}$. Then, the \ac{RHS} of \eqref{eq:SC_bound} can be computed via $\ell^{(i)}_{\G^{(m)}}$ with $i = 1,\dots,k$, i.e., as
\[\sum_{i=1}^{k}\lim\limits_{z\rightarrow 0} \left(\int_{-\infty}^{-z}\ell^{(i)}_{\G^{(m)}}(x)dx+\frac{1}{2}\int_{-z}^{+z}\ell^{(i)}_{\G^{(m)}}(x)dx\right).\]
An efficient method to compute such an expression is quantized density evolution \cite{chung_urbanke2001}.%Using this approach, the \ac{RHS} of \eqref{eq:DE_upper_bound} is computed. Its tightness is numerically demonstrated in Sec. \ref{sec:numerical_results}.


==> numerical_results.tex <==
%\section{Numerical Results}
%\label{sec:numerical_results}

\iffalse
\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.75\columnwidth]{./figures/125_64_SPC_document_polar_BEC.pdf}
	\end{center}
	\vspace{-0.5cm}
	\caption{\ed{\ac{CER} vs. \ac{SNR}  under \ac{SCL} decoding for a $(125,64)$ product code with various list sizes, compared to a $(125,64)$ polar code with various list sizes.}
	}\label{fig:scl_125_64_SPC_vs_polar}
\end{figure}

\ed{Next, we provide simulation results for the $3$-dimensional $(125,64)$ \ac{SPC} product code under \ac{SCL} decoding with various list sizes in Fig. \ref{fig:scl_125_64_SPC_vs_polar}. As reference, simulation results for a $(125,64)$ punctured polar code~\cite{WR14:polar_punc} is also provided. Note that the design follows the guidelines of 5G standard~\cite{BCL21:5g_polar}. In addition, the \ac{TSB} (a tight upper bound on the error probability for a given code under \ac{ML} decoding~\cite{poltyrev94}) is also provided.} Remarkably, \ed{\ac{SCL}} decoding with $L=4$ is sufficient to operate on top of the \ac{TSB} and outperform \ac{BP} decoding. With $L=8$, the \ac{SCL} decoder tightly matches the \ac{ML} lower bound, which is not the case for \ac{BP} decoding. The gap to the \ac{RCU} bound reaches to \ed{$1.7$} dB at \ac{CER} of $10^{-3}$. \ed{When $L=4$ is considered, the gap to the performance of polar code is around $0.3$ dB at \ac{CER} of $10^{-3}$ and note also that the polar code performs significantly better under \ac{SC} decoding since its set $\mathcal{A}$ is chosen to minimize the \ac{CER} under \ac{SC} decoding.}
\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.75\columnwidth]{./figures/125_64_SPC_document_polar.pdf}
	\end{center}
	\vspace{-0.5cm}
	\caption{\ed{\ac{CER} vs. \ac{SNR}  under \ac{SCL} decoding for a $(125,64)$ product code with various list sizes, compared to a $(125,64)$ polar code with various list sizes.}
	}\label{fig:scl_125_64_SPC_vs_polar}
\end{figure}

\iffalse
\ed{Fig. \ref{fig:scl_125_58_SPC} shows the performance of concatenating the $(125,64)$ product code with \ed{a $6$-bit} outer \ac{CRC} code with generator polynomial $g(x)=x^6+x+1$, where the interleaver between the codes is the trivial one defined by an identity matrix. This concatenation leads to a $(125,58)$ code. Since the code distance properties are improved (observed directly via the \ac{TSB} on the average performance of the code ensemble), the performance improvement under \ac{ML} decoding is expected to be significant. The gain achieved by \ac{SCL} decoding is remarkably large, operating below the \ac{TSB}. At  a \ac{CER} range of $10^{-2}$-$10^{-4}$, \ac{SCL} decoding of the concatenated code achieves gains up to $1.25$ dB over the original product code. The gap to the \ac{RCU} bound is approximately $0.7$ dB at the \ac{CER} of $10^{-3}$ and reaching up to $1$ dB at the \ac{CER} of $10^{-4}$. Note that it is not always possible to attain the performance close to the \ac{ML} performance of concatenated codes using \ac{BP} decoding\cite{Coskun19:RM-Product,geiselhart2020crcaided}. In that sense, \ac{SCL} decoding provides a low-complexity solution to reach the \ac{ML} performance of the concatenated scheme.}
\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.75\columnwidth]{./figures/125_64_bestCRC6_SPC_document.pdf}
	\end{center}
	\vspace{-0.5cm}
	\caption{\ac{CER} vs. \ac{SNR}  under \ac{SCL} decoding for a $(125,64)$ product code concatenated with a $(64,58)$ \ac{CRC} code, with various list sizes. It is compared to a $(125,56)$ CRC-concatenated polar code with various list sizes, where the generator polynomial of the outer code is optimized for \ac{SCL} decoding\cite{Yuan19}.
	}\label{fig:scl_125_58_SPC}
\end{figure}
\fi

Fig. \ref{fig:scl_125_56_SPC} shows the performance of concatenating the $(125,64)$ product code with \ed{a $8$-bit} outer \ac{CRC} code with generator polynomial \ed{$g(x)=x^8+x^6+x^5+x^4+x^2+x+1$}, where the interleaver between the codes is the trivial one defined by an identity matrix. This concatenation leads to a $(125,56)$ code. Since the code distance properties are improved (observed directly via the \ac{TSB} on the average performance of the code ensemble), the performance improvement under \ac{ML} decoding is expected to be significant. The gain achieved by \ac{SCL} decoding is remarkably large, operating below the \ac{TSB} \ed{obtained for the average weight enumerator of a concatenated ensemble with the uniform distribution assumption over all possible interleavers.}. At  a \ac{CER} of $10^{-2}$, \ac{SCL} decoding of the concatenated code achieves gains up to $1.25$ dB over the original product code, reaching up to \ed{$1.5$} dB at a \ac{CER} $\approx 10^{-4}$. The gap to the \ac{RCU} bound is approximately \ed{$0.7$} dB at the \ac{CER} of \ed{$10^{-4}$ and less for lower \acp{CER}, providing a competitive performance for similar parameters\cite{Coskun18:Survey}}. Note that it is not always possible to attain the performance close to the \ac{ML} performance of concatenated codes using \ac{BP} decoding\cite{Coskun19:RM-Product,geiselhart2020crcaided}. In that sense, \ac{SCL} decoding provides a low-complexity solution to reach the \ac{ML} performance of the concatenated scheme. \ed{As a reference, a (125, 56) CRC-concatenated polar code is constructed by using the $(125,64)$ polar code of Fig. \ref{fig:scl_125_56_SPC} with an $8$-bit outer \ac{CRC} code optimized using the guidelines of \cite{Yuan19}. The generator polynomial for the CRC code is $f(x)=x^8+x^7+x^6+x^5+1$. Note that the gap to the \ac{ML} performance of two codes is less than $0.5$ dB in the considered regime.\footnote{\ed{A careful optimization of the interleaver for the CRC-concatenated \ac{SPC} product code might provide further gains, but it is not in the scope of this work.}}}
\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.75\columnwidth]{./figures/125_64_bestCRC8_SPC_document.pdf}
	\end{center}
	\vspace{-0.5cm}
	\caption{\ac{CER} vs. \ac{SNR}  under \ac{SCL} decoding for a $(125,64)$ product code concatened with a $(64,56)$ \ac{CRC} code, with various list sizes.  \ed{It is compared to a $(125,56)$ CRC-concatenated polar code with various list sizes, where the generator polynomial of the outer code is optimized for \ac{SCL} decoding\cite{Yuan19}.}
	}\label{fig:scl_125_56_SPC}
\end{figure}
\fi
